Mid-J CO shock tracing observations of infrared dark clouds II Low-J CO constraints on excitation, depletion, and kinematics

Infrared dark clouds are kinematically complex molecular structures in the interstellar medium that can host sites of massive star formation. We present 4 square arcminute maps of the 12CO, 13CO, and C18O J = 3 to 2 lines from selected locations within the C and F (G028.37+00.07 and G034.43+00.24) infrared dark clouds (IRDCs), as well as single pointing observations of the 13CO and C18O J = 2 to 1 lines towards three cores within these clouds. We derive CO gas temperatures throughout the maps and find that CO is significantly frozen out within these IRDCs. We find that the CO depletion tends to be the highest near column density peaks, with maximum depletion factors between 5 and 9 in IRDC F and between 16 and 31 in IRDC C. We also detect multiple velocity components and complex kinematic structure in both IRDCs. Therefore, the kinematics of IRDCs seem to point to dynamically evolving structures yielding dense cores with considerable depletion factors.

==> test.tex <==
VIEW={DEFAULT}
  COO=0.500000 0.500000 0.500000
  C2C=0.10240529477596283 0.4266226291656494 -0.8986135125160217
  ROO=2.5
  ROLL=16.399794753841075
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
END



==> test2.tex <==
VIEW={DEFAULT}
  COO=0.500000 0.500000 0.500000
  C2C=-0.19919359683990479 0.5437154173851013 -0.8152884840965271
  ROO=3.0
  ROLL=-21.895264214743076
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
END


